Leveraging Human Salience to Improve Calorie Estimation

The following paper investigates the effectiveness of incorporating human salience into the task of calorie prediction from images of food. We observe a 32.2% relative improvement when incorporating saliency maps on the images of food highlighting the most calorie regions. We also attempt to further improve the accuracy by starting the best models using pre-trained weights on similar tasks of mass estimation and food classification. However, we observe no improvement. Surprisingly, we also find that our best model was not able to surpass the original performance published alongside the test dataset, Nutrition5k. We use ResNet50 and Xception as the base models for our experiment.

==> chapters/future.tex <==
Given that the ability to correctly identify foods and use their mass is crucial to the success of humans at predicting calories, our results that pre-training the model on these tasks did not improve the predictions is surprising. One possible way to better utilize these pre-trained models is to combine them into an ensemble model. Before finalizing this project, we hope to compare the results of such an ensemble model to the results presented in the current paper. We also hope to compare the best models resulting from our experiments against those published with the test dataset we've been using, Nutrtion5k \cite{thames2021nutrition5k}. In their experiments, they trained and tested models on the same dataset which we did not do. We aim to take our best models and fine-tune them with the same train set as the original authors. Finally, using the same test set we can compare our models against theirs. Their baseline models achieve a MAE of 150.8, although they also provide other models which incorporate depth and mass information which achieve as little as 24.1 MAE.  
